Heavy-tailed Representations, Text Polarity Classification & Data Augmentation

The dominant approaches to text representation in natural language rely on learning embeddings on massive corpora which have convenient properties such as compositionality and distance preservation. In this paper, we develop a novel method to learn a heavy-tailed embedding with desirable regularity properties regarding the distributional tails, which allows to analyze the points far away from the distribution bulk using the framework of multivariate extreme value theory. In particular, a classifier dedicated to the tails of the proposed embedding is obtained which performance outperforms the baseline. This classifier exhibits a scale invariance property which we leverage by introducing a novel text generation method for label preserving dataset augmentation. Numerical experiments on synthetic and real text data demonstrate the relevance of the proposed framework and confirm that this method generates meaningful sentences with controllable attribute, e.g. positive or negative sentiment.

==> backuo.tex <==
\iffalse
\begin{table}[ht]
\scriptsize
    \centering
    
        \begin{tabular}{|c|cc|cc|}
       \hline \multirow{2}{*}{} & \multicolumn{2}{c|}{\textit{Amazon}} & \multicolumn{2}{c|}{\textit{Yelp}}\\
        & dataset 1 & dataset 2        & dataset 1 & dataset 2 \\\hline
          $\vert \mathcal{D}_n^{Train} \vert$ &750  & 210k & 750 & 1400k\\
          $\vert \mathcal{D}_n^{Test} \vert$ & 250 & 22k & 250 & 22k \\
    $\vert\mathcal{T}_{\text{test}}\vert$ & 61 & 6.9k  & 97 & 6.1k\\\hline
%            \multirow{2}{*}{} & \multicolumn{2}{c|}{\textit{Yelp}} \\
%        & dataset 1 & dataset 2 \\\hline
%        $\vert \mathcal{D}_n^{Train} \vert$ & 750 & 1,400k\\
%         $\vert \mathcal{D}_n^{Test} \vert$ & 250 & 22k \\
%    $\vert\mathcal{T}_{\text{test}}\vert$ & 97 & 6,1k\\\hline
    \end{tabular}
    \caption{Sizes of the train  $\mathcal{D}_n^{Train}$, test $\mathcal{D}_n^{Test}$ and the extreme test set $\mathcal{T}_{\text{test}}$. The extreme train tests constitute $1/4$ of the  full train tests. These datasets are used to validate  {\fontfamily{qcr}\small\textbf{LHTR}}.}
    %\addedp{faut utiliser des mid rules pour les traits horizontaux des tableau c'est moche}
    \label{tab:my_label}
\end{table}
\fi




The three competing methods obtain the exact same scores on \textit{Amazon small dataset } (Figure~\ref{fig:small_yelp}), which may possibly be explained by the fact that the classification task is known to be easy on this dataset. Indeed, the two classes are well separated in the three representations except for rare counter-examples, leading to identical performances. 

%even though the improvement is moderate  on the  small size dataset \textit{Amazon dataset~1}


\begin{subfigure}[t]{0.22\textwidth}
\includegraphics[width=1\textwidth]{figures/small_datasets/small_amazon/hamming_loss_extreme_amazon.pdf}
\caption{}
  \label{fig:small_amazon}
\end{subfigure}
\begin{subfigure}[t]{0.22\textwidth}
  \includegraphics[width=\textwidth]{figures/small_datasets/small_yelp/hamming_loss_extreme_yelp.pdf}
  \caption{}
  \label{fig:small_yelp}
\end{subfigure}
Table~\ref{tab:my_label} summarizes the sizes of the used datasets together with the proportion of training and testing data used in our experiments. Note that each sample 

==> explanabilite_bak.tex <==
\section{Extremes in Text}

\addeda{pour toute la section, pouvez-vous faire attention à faire correctement reference aux figures? comme parfois on n'arrive pas à lire les axes je n'arrive pas à comprendre quelle figure regarder pour les différents points de l'argumentaire. par exemple il n'y a pas de figure 14.}
\\~\\

\addeda{ Pas mal de figures (boxplots et histogrammes) pourraient être supprimées et remplacées simplement par des pairwise plots des trois quantités suivantes (sans séparer les extremes et les non extremes car cette separation est arbitraire, à force vous avez compris): \\
1) norme dans la représentation BERT \\2) norme dans la representation \HTalgo \\3) longueur de la phrase.\\~\\ Parce qu'une maniere de resumer la discussion est : \\
 (i)   les trois grandeurs ci-dessus sont corrélées positivement \\  (ii) les phrases plus longues/ de grande norme dans \HTalgo / de grande norme dans BERT  sont plus difficiles à classer. 
 \\~\\
 En fait , pour synthetiser encore, je crois qu'on a simplement une corrélation positive entre les trois grandeurs ci-dessus et la quatrième (binaire): 4): mauvaise classification de la phrase par BERT.   \\~\\
 Si ce discours tient la route on a donc la magnigfique  histoire suivante à raconter:  \\
 0) il y a des queues  épaisses dans le texte naturel mais pas dans BERT, c'est louche. \\
 1) les extremes (grande norme) de BERT sont plus durs à classifier  \\
 %(un pairwise plot ici est équivalent à deux boxplot de la norme des phrases dans bert, avec un boxplot pour les phrases bien classées et un boxplot pour les phrases mal classées (boxplot ou histogramme d'ailleurs, peu importe)  \\
 3) les extremes de  BERT sont aussi (en probabilité) les extremes de LHTR 
 4) Avec EVT on est capables de mieux classer ces extremes \\~\\
} 
 % pour les pairwise plots, tu pensais à ça : https://seaborn.pydata.org/generated/seaborn.pairplot.html 
 % par exemple. enfin le plot des paires X_i en abscisse, X_j en ordonnée, pour i <  j (donc sans la diagonale inutile de seaborn) avec 3 ou 4 variables y a pas tant de paires que ça, faites le à la main. 
 % ok ok
 % bon la petite mamie va se coucher, à demain 
 %% haha bonne soirée :)
 
The aim of this section is to provide some intuition on what characterizes samples falling in the extreme region of \HTalgo.
Concretely we show that ($i$) the length of the sentences tends to be longer for points belonging to the extreme set, ($ii$) our experiments hint that the norm of the extreme points tends to be larger and that this phenomenon cannot only be explained by the fact that longer sentences have larger embedding norms through BERT \addeda{ ce dernier 'fact' est-il un truc connu? ou est-ce que vous le montrez? }
%\addeda{ je comprends pas  ce que ça veut dire 'longer embedding through BERT' puisque on parle de vecteur. plutôt 'larger norm' ? }, 
Finally we hypothesize that the extremes from \HTalgo\ %\addeda{ in which representation? } 
are samples that are harder to model for a language model based on BERT. 

\subsection{Sentences lying in the extreme regions of \HTalgo\ are longer}\label{subsection:extremes_longer}
We observe (see histograms in Figure~\ref{fig:lengrh}) that for both \textit{Yelp} and \textit{Amazon} datasets, extremes from \HTalgo\ contain on average significantly more words than the non extreme samples for both label classes. \textit{An extreme sentence is more likely to be a long sentence}. This result is reinforced by %boxplots from Figure~\ref{fig:boxplot__amazon__yelp} and 
Kolmogorov-Smirnoff tests between the length distributions of the two considered class for each label. The tests allow to reject the null hypothesis of equality between distributions, as the maximum $p$-values is smaller than  $0.05$.
\begin{figure}[H]
\centering
\begin{subfigure}[t]{0.45\textwidth}
    \includegraphics[width=\textwidth]{figures/yelp_distribution_+1.pdf}
    \caption{\textit{Yelp} - labeled $+1$ }
    \label{fig:Yelp+1}
\end{subfigure}
\begin{subfigure}[t]{0.45\textwidth}
    \includegraphics[width=\textwidth]{figures/yelp_distribution_-1.pdf}
    \caption{\textit{Yelp} -  labeled $-1$ }
    \label{fig:Yelp-1}
\end{subfigure}

\begin{subfigure}[t]{0.45\textwidth}
    \includegraphics[width=\textwidth]{figures/amazon_distribution_+1.pdf}
    \caption{\textit{Amazon} -  labeled $+1$ }
    \label{fig:Amazon+1}
\end{subfigure}
\begin{subfigure}[t]{0.45\textwidth}
    \includegraphics[width=\textwidth]{figures/amazon_distribution_-1.pdf}
    \caption{\textit{Amazon} - labeled $-1$}
    \label{fig:Amazon-1}
\end{subfigure}
\caption{Histograms of the samples' sentence length for \textit{Yelp} dataset (Figure~\ref{fig:Yelp+1} and Figure~\ref{fig:Yelp-1}) and \textit{Amazon}  (Figure~\ref{fig:Amazon+1} and Figure~\ref{fig:Amazon-1}). The number of sentences in the bulk is approximately $3$ times the number of extreme sentences for each dataset $10000$ sentences are considered and extreme region contains approximately $3000$ sentences.}
\label{fig:lengrh}
\end{figure}

\iffalse
\begin{figure}[h]
    \centering
    \includegraphics[width=0.45\textwidth]{figures/boxplotamazon.pdf}
    \includegraphics[width=0.45\textwidth]{figures/boxplotyelp.pdf}
    \caption{Boxplot of samples' sentence length for \textit{Amazon} and \textit{Yelp} datasets for both regions and both labels.}
    \label{fig:boxplot__amazon__yelp}
\end{figure}
\fi

To illustrate the variation of the sequence length in the extreme regions we consider nested  subsets of the extreme  test set $\mathcal{T}_{\text{test}}$,  $\mathcal{T^\lambda} = \{z \in \mathcal{T}_{\text{test}},  \|z\| \geq \lambda t\}$, $\lambda\ge 1$. For all factor $\lambda \geq 1 $, $\mathcal{T^\lambda} \subseteq \mathcal{T}_{\text{test}}$. The greater $\lambda$, the fewer the samples retained for evaluation and the greater their  norms. In Figure~\ref{fig:boxplot_length}) we report the variation of the sequence lengths for the aforementioned nested sets. \textit{The more extreme the longer the sentences.} 
\begin{figure}[h]
    \includegraphics[width=\textwidth]{explanibility/length_yelp.pdf}\caption{Yelp}\label{fig:yelp_length}
    \includegraphics[width=\textwidth]{explanibility/length_amazon.pdf}\caption{Amazon}\label{fig:amaon_length}
    \caption{Boxplot of Sentence length for  \textit{Yelp} (Fig~\ref{fig:yelp_length}) \textit{Amazon} (Fig~\ref{fig:amaon_length}) on the bulk and the extreme region.}
    \label{fig:boxplot_length}
\end{figure}

\subsection{Sentences lying in the extreme regions of \HTalgo\ tend to have greater norms when embedded with BERT }\label{subsection:extremes_norms}
In this section, we study the evolution of the norm of representations for sentences with BERT embedding. The considered norm is the infinite norm. To illustrate the variation of the norm in the extreme regions we consider nested subsets of the extreme test set based on representations from \HTalgo.  We observe (see boxplots in Figure~\ref{fig:boxplot_norm}) for both \textit{Yelp} and \textit{Amazon} datasets, that extremes from \HTalgo\ have greater norm with BERT embedding than the non extreme samples. \textit{An extreme sentence with \HTalgo\ embedding is more likely to have a greater norm with BERT embedding}.
\begin{figure}[h]
    \centering
    \includegraphics[width=\textwidth]{explanibility/norm_yelp.pdf}\caption{Yelp}\label{fig:yelp_norm}
    \includegraphics[width=\textwidth]{explanibility/norm_amazon.pdf}\caption{Amazon}\label{fig:amaon_norm}
    \caption{Boxplot of norm for sentences embedded with BERT for  \textit{Yelp} dataset (Fig~\ref{fig:yelp_norm}) abd \textit{Amazon} dataset (Fig~\ref{fig:amaon_norm}) on the bulk and the extreme region from \HTalgo.}%We consider the infinity norme.
    \label{fig:boxplot_norm}
\end{figure}

To reinforce that the norms difference between embeddings from BERT, as observed in Figure \ref{fig:boxplot_norm}, is not only due to longer extreme sentences -resulting in embeddings with greater norms- we report in Figure~\ref{fig:boxplot_norm_length} the length of the sentence as a function of the infinite norm of the sentence representation with BERT embedding.
\begin{figure}[h]
    \centering
        \centering
    \begin{subfigure}[t]{0.45\textwidth}
    \includegraphics[width=\textwidth]{explanibility/bert_norm_yelp.pdf}
    \caption{\textit{Yelp}}
    \label{fig:yelp_norm_length}
    \end{subfigure}
    \begin{subfigure}[t]{0.45\textwidth}
        \includegraphics[width=\textwidth]{explanibility/bert_norm_amazon.pdf}
        \caption{\textit{Amazon}}
        \label{fig:amaon_norm_lenght}
    \end{subfigure}
    \caption{Evolution of sentence length as a function of its embedding norm using BERT for \textit{Yelp} (Fig~\ref{fig:amaon_norm_lenght}) \textit{Amazon} (Fig~\ref{fig:amaon_norm_lenght}) on the bulk and the extreme regions computed with \HTalgo.}%. We consider the infinity norm.
    \label{fig:boxplot_norm_length}
\end{figure}


\clearpage
\subsection{Are extreme samples harder to model for BERT? }\label{subsection:modelling}

In the classification experiment in Section \ref{sec:classifExtremes}, we saw that a classifier trained on BERT is outperformed by an equivalent trained on \HTalgo. We make the hypothesis that this could result from longer sentences (like the ones encountered in the extreme regions) are harder to model for BERT. Figure~\ref{fig:boxplot_lm} illustrates the next token prediction loss for a Language model trained on BERT for both samples from both extreme and bulk computed on \HTalgo. Result show that BERT is more uncertain on extreme sample 
%\addeda{pas une phrase. pourquoi 'although'? }
%\addeda{Heu ... je ne vois pas de différence, quant à la moyenne, et malheureusement la variance est plus grande sur le bulk que sur les extremes. vous avez tracé un coût ou un score ? (c'est mieux d'avoir des petites ou des grandeds valeurs? }
\addeda{préciser qu'on ne voit rien sur yelp, à part malheureusement une plus grande variance sur le bulk. on constate le phenomene seulement sur amazon.}
When truncating sentences to $60$ words we observe that this difference tends to vanish \addeda{on ne voit pas de différence  à l'oeil nu, entre les figures amazon tronquées ou non (encore moins sur yelp)} meaning that the length is probably the main factor
%%\addeda{au contraire sur la figure du bas on voit une différence, mais pas sur la figure du haut.}. % long range dependencies. 

%% Erreur de sauvegarde celui la il est pas bon :) 
%% (anne) c'est pas la bonne figure? non :/ 
\begin{figure}[h]
    \centering
    \includegraphics[width=\textwidth]{explanibility/next_token_yelp.pdf}\caption{Yelp}\label{fig:yelp_next}
    \includegraphics[width=\textwidth]{explanibility/next_token_amazon.pdf}\caption{Amazon}\label{fig:amaon_next}
    \caption{Boxplot of Norm for the next token prediction loss for a LM trained on BERT  \textit{Yelp} (Fig~\ref{fig:yelp_next}) \textit{Amazon} (Fig~\ref{fig:amaon_next}) on the bulk and the extreme region.}
    \label{fig:boxplot_lm}
\end{figure}
\addeda{les captions/label dans des sous figures font bugger les ref croisees. utilisez 'Figure n-top / Figure n-bottom' plutôt; en plus la figure ci-dessus et ci-dessous ont le même label}

\addeda{et mais vous avez mis deux fois la meme figure ! forcément on ne voit rien !!}
%% Erreur de sauvegarde celui la il est pas bon :) 
\begin{figure}[h]
    \centering
    \includegraphics[width=\textwidth]{explanibility/next_token_yelp.pdf}\caption{Yelp}\label{fig:yelp_next}
    \includegraphics[width=\textwidth]{explanibility/next_token_amazon.pdf}\caption{Amazon}\label{fig:amaon_next}
    \caption{Boxplot for the next token prediction loss for a LM trained on BERT all sentences have been truncated to $60$ \textit{Yelp} (Fig~\ref{fig:yelp_next}) \textit{Amazon} (Fig~\ref{fig:amaon_next}) on the bulk and the extreme region.}
    \label{fig:boxplot_lm}
\end{figure}

